Introducing HiggsBounds 2.0.0

We introduce version 2.0.0 of the computer program HiggsBounds. The program tests neutral and charged Higgs sectors of new models against the current exclusion bounds from LEP and the Tevatron. As input, it requires a selection of model predictions, such as Higgs masses, branching ratios, effective couplings and total decay widths. The program then uses the expected and observed topological cross section limits from the Higgs searches to determine whether a given parameter scenario of a model is excluded at the 95% C.L. by those searches. Version 2.0.0 includes 39/53 LEP/Tevatron Higgs search analyses, compared to 13/36 in the previous release (1.2.0). Among the newly included analyses are LEP searches for neutral Higgs bosons (H) decaying invisibly or into hadrons, LEP searches via the production modes (tau+ tau- H) and (b b-bar H), Tevatron searches via (t t-bar H), and LEP and Tevatron searches for charged Higgs bosons. Also, all Tevatron results presented at the ICHEP'10 are included in version 2.0.0. In this talk, we explain the basic ideas behind the implementation of HiggsBounds and provide a list of search topologies implemented in version 2.0.0. Furthermore, we apply HiggsBounds 2.0.0 to (a) determine the allowed Higgs mass range for a simple 4th generation model, (b) update/reproduce LEP/Tevatron Higgs exclusion plots for the MSSM m_h-max benchmark scenario, and (c) show exclusion results for the scalar sector of the Randall-Sundrum model.

==> preprint.tex <==
BONN-TH-2010-14, DESY 11-006, FR-PHENO-2010-044

